Causal Bayesian Optimization

This paper studies the problem of globally optimizing a variable of interest that is part of a causal model in which a sequence of interventions can be performed. This problem arises in biology, operational research, communications and, more generally, in all fields where the goal is to optimize an output metric of a system of interconnected nodes. Our approach combines ideas from causal inference, uncertainty quantification and sequential decision making. In particular, it generalizes Bayesian optimization, which treats the input variables of the objective function as independent, to scenarios where causal information is available. We show how knowing the causal graph significantly improves the ability to reason about optimal decision making strategies decreasing the optimization cost while avoiding suboptimal solutions. We propose a new algorithm called Causal Bayesian Optimization (CBO). CBO automatically balances two trade-offs: the classical exploration-exploitation and the new observation-intervention, which emerges when combining real interventional data with the estimated intervention effects computed via do-calculus. We demonstrate the practical benefits of this method in a synthetic setting and in two real-world applications.

==> case_studies.tex <==
%%%%%%%%%
\subsection{Case studies}
The \cbo setting can be found in a variety of fields and decision making problems ranging from system optimisation to clinical trials or public policy design, just to cite a few. Here we present two of such settings that will be then analysed in the following experimental session. 
%medical drug testing
%policy settings 

\paragraph{\experiment 1: Synthetic setting}
The first application consists in an example shown in (\cite{cochran1957experimental}) in which $\mat{Y}$ denotes the crop yields for different agricultural products, $X_1$ represents the level of fumigants, $X_2$ denotes the eelworm population while $X_3$ captures the population of birds and other predators. $\mat{C}$ represents the set of non-manipulative variables.  \fig \ref{fig:dag_related_methods} (lower \DAG) represents the investigator's understanding of the major causal influences on crop yields. We wish to find the set of interventional variables and values leading to the highest yield in a limited number of seasons. In this case, we assume the same graphical graph for all outcome variables. A similar analysis can be repeated for multiple Y with different target functions and does looking at the multi objective optimisation. 

\paragraph{\experiment 2: System Optimization}
The second application considers the problem of supply chain optimisation within a company. A supply chain is a network of facilities that procure raw materials, transform them into the final goods and delivers the products to costumers.  Bayesian networks have been successfully used in this field \virgi{add references} to monitor performances at different stages and ensure efficient operations. Nowadays, optimising the system is made more challenging by the size and complexity of many real-world supply chains, combined with their dynamic and stochastic nature, see \fig .. for an example. 
%%%%%%%%


==> causal_graph.tex <==
\begin{figure}[h!]
  \centering
  \tikz{ %
   \node[obs] (X_1) {$X_1$} ; %
    \node[obs,below left= of X_1] (X_2) {$X_2$} ; %
    \node[obs, below right=of X_1](Y){$\mat{Y}$}; %
        \node[obs, right = of Y] (X_3) {$X_3$} ; %
        \node[obs, above left = of X_3] (C) {$\mat{C}$} ; %
    \edge {X_1} {Y} ; %
     \edge {X_2} {Y} ; %
      \edge {X_3} {Y} ; %
       \edge {X_1} {X_2} ; %
       \edge {C} {X_2} ;
       \edge {C} {X_3} ;
        \edge {C} {Y} ;
  }
\caption{\DAG for \experiment 1.}
\label{fig: DAG}
\end{figure}

==> panel.tex <==
\begin{figure*}
    \centering
    %% PANEL A
    \begin{subfigure}[t]{0.3\textwidth}
       \centering
       \tikz{ %
       	\node[obs] (X) {$X$} ; %
       	\node[obs, right = of X, xshift=0.2cm] (Z) {$Z$} ; %
       	\node[obs, right = of Z] (Y) {$Y$} ; %
       	\edge {X} {Z} ; %
       	\edge {Z} {Y} ; %
       	
       	\node[rectangle, below=-0.2cm, text width=3cm, below = of Z, yshift=1.2cm, xshift=-0.9cm] (eq) {
       		\begin{align*}
       		X &=  \epsilon_X \\
       		Z &= \exp(-X) + \epsilon_Z\\
       		Y & = \text{cos}(Z) - \exp(-Z/20) + \epsilon_Y
       		\end{align*}} ; %	
       	\node[rectangle, draw, below=-0.2cm, text width=3.5cm, below = of eq, yshift=1.cm, xshift=0.9cm] (eq2) {\mis = \{$\emptyset$, $\{X\}$, $\{Z\}$\} \\ \pomis = \{$\{Z\}$\}} ; %
       }
   \label{fig:toy_model}
    \end{subfigure}
%% PANEL B
    \begin{subfigure}[t]{0.3\textwidth}
	\centering
	\vspace{-3.5cm}
	\includegraphics[width=1.0\linewidth]{images/intervention_XandZ.png} 
	\includegraphics[width=0.5\linewidth]{images/intervention_X_Z.png} 
    \end{subfigure}
%% PANEL C
   \begin{subfigure}[t]{0.3\textwidth}
	\centering
	\vspace{-3.7cm}
		\includegraphics[width=1.0\linewidth]{images/model_no_mf.png} 
	\includegraphics[width=1.\linewidth]{images/model_mf.png} 
\end{subfigure}

    \vspace{0.1cm}
    \begin{subfigure}[t]{0.3\textwidth}
        \centering
        	\vspace{-3.7cm}
%        \begin{forest}
%        	[{\includegraphics[width=0.5\linewidth]{images/convex_hull.png}} $\alpha$
%        	[$\emptyset$
%        	]
%        	[ $\{\{X\}\text{,}\{X\}\}$
%        	[{\includegraphics[width=0.5\linewidth]{images/acquisition.png}}
%        	]
%        	]
%        	]
%        \end{forest}
	\includegraphics[width=1.\linewidth]{images/convex_hull.png} 
\includegraphics[width=1.0\linewidth]{images/acquisition.png} 
    \end{subfigure}
%% PANEL E
     \begin{subfigure}[t]{0.3\textwidth}
     	\centering
     	\vspace{-3.7cm}
     	\includegraphics[width=1.\linewidth]{images/model_no_mf_final.png} 
    		\includegraphics[width=1.0\linewidth]{images/model_mf_final.png} 
    \end{subfigure}
%% PANEL D
    \begin{subfigure}[t]{0.3\textwidth}
    	\centering
       \includegraphics[width=1.\linewidth]{images/X_Y_Z_Cost_X.png} 
    \end{subfigure}
    \caption{Some general caption of all the figures. In (\subref{fig:timing1}) you can see a  green square....}
\end{figure*}

==> related.tex <==
\section{Related work}

==> toy_example.tex <==
%% Panel A
\begin{figure}
	\centering
	~ %add desired spacing between images, e. g. ~, \quad, \qquad etc.
	%(or a blank line to force the subfigure onto a new line)
		\centering
		\tikz{ %
			\node[obs] (X) {$X$} ; %
			\node[obs, right = of X, xshift=0.2cm] (Z) {$Z$} ; %
			\node[obs, right = of Z] (Y) {$Y$} ; %
			\edge {X} {Z} ; %
			\edge {Z} {Y} ; %
			
			\node[rectangle, below=-0.2cm, text width=3cm, below = of Z, yshift=1.2cm, xshift=-0.9cm] (eq) {
					\begin{align*}
					X &=  \epsilon_X \\
					Z &= \exp(-X) + \epsilon_Z\\
					Y & = \text{cos}(Z) - \exp(-Z/20) + \epsilon_Y
					\end{align*}} ; %	
				\node[rectangle, draw, below=-0.2cm, text width=3.5cm, below = of eq, yshift=1.cm, xshift=0.9cm] (eq2) {\mis = \{$\emptyset$, $\{X\}$, $\{Z\}$\} \\ \pomis = \{$\{Z\}$\}} ; %
		}
\end{figure}



